Sketching Word Vectors Through Hashing

We propose a new fast word embedding technique using hash functions. The method is a derandomization of a new type of random projections: By disregarding the classic constraint used in designing random projections (i.e., preserving pairwise distances in a particular normed space), our solution exploits extremely sparse non-negative random projections. Our experiments show that the proposed method can achieve competitive results, comparable to neural embedding learning techniques, however, with only a fraction of the computational complexity of these methods. While the proposed derandomization enhances the computational and space complexity of our method, the possibility of applying weighting methods such as positive pointwise mutual information (PPMI) to our models after their construction (and at a reduced dimensionality) imparts a high discriminatory power to the resulting embeddings. Obviously, this method comes with other known benefits of random projection-based techniques such as ease of update.

==> parameters/old-2+2+various-s-men.tex <==
1	3000	� 	�	�	0.7371	0.7341	0.7389
2	3000	� 	�	�	0.7288	0.7255	0.7322
3	3000	� 	�	�	0.7191	0.7162	0.7205
4	3000	� 	�	�	0.7105	0.7052	0.7158
5	3000	� 	�	�	0.7083	0.7041	0.7132
6	3000	� 	�	�	0.7025	0.699	0.7067
7	3000	� 	�	�	0.6937	0.6883	0.6997
8	3000	� 	�	�	0.6943	0.6903	0.7032
9	3000	� 	�	�	0.6927	0.6891	0.6989
10	3000	� 	�	�	0.6878	0.6833	0.6953
11	3000	� 	�	�	0.6845	0.6806	0.6876
12	3000	� 	�	�	0.6809	0.6658	0.6884
13	3000	� 	�	�	0.6836	0.6807	0.688
14	3000	� 	�	�	0.6756	0.6657	0.6826
15	3000	� 	�	�	0.6749	0.6723	0.6774
16	3000	� 	�	�	0.6749	0.6711	0.6787
17	3000	� 	�	�	0.6735	0.6684	0.6777
18	3000	� 	�	�	0.6731	0.6689	0.6774
19	3000	� 	�	�	0.6679	0.6629	0.6716
20	3000	� 	�	�	0.6686	0.6665	0.6704
21	3000	� 	�	�	0.6642	0.6619	0.6679
22	3000	� 	�	�	0.6643	0.6601	0.6684
23	3000	� 	�	�	0.661	0.6504	0.6675
24	3000	� 	�	�	0.6618	0.6542	0.6702
25	3000	� 	�	�	0.6643	0.6529	0.6702
26	3000	� 	�	�	0.658	0.6485	0.6626
27	3000	� 	�	�	0.6564	0.653	0.6601
28	3000	� 	�	�	0.6571	0.6503	0.6658
29	3000	� 	�	�	0.653	0.6444	0.6575

==> pop <==
@inproceedings{Agirre2009,
 author = {Agirre, Eneko and Alfonseca, Enrique and Hall, Keith and Kravalova, Jana and Pasca, Marius and Soroa, Aitor},
 title = {A Study on Similarity and Relatedness Using Distributional and WordNet-based Approaches},
 booktitle = {HLT-NAACL '09},
 year = {2009},
 isbn = {978-1-932432-41-1},
 location = {Boulder, Colorado},
 pages = {19--27},
 numpages = {9},
 url = {http://dl.acm.org/citation.cfm?id=1620754.1620758},
 acmid = {1620758},
 publisher = {ACL},
 address = {Stroudsburg, PA, USA},
}


@article{LemkeOliver02082016,
author = {Lemke Oliver, Robert J. and Soundararajan, Kannan}, 
title = {Unexpected biases in the distribution of consecutive primes},
volume = {113}, 
number = {31}, 
pages = {E4446-E4454}, 
year = {2016}, 
doi = {10.1073/pnas.1605366113}, 
URL = {http://www.pnas.org/content/113/31/E4446.abstract}, 
eprint = {http://www.pnas.org/content/113/31/E4446.full.pdf}, 
journal = {Proceedings of the National Academy of Sciences} 
}

@InProceedings{AroraBGM14,
  Title                    = {Provable Bounds for Learning Some Deep Representations},
  Author                   = {Arora, Sanjeev and Bhaskara, Aditya and Ge, Rong and Ma, Tengyu},
  Booktitle                = {{ICML} 2014, Beijing, China, 21-26 June 2014},
  Year                     = {2014},
  Pages                    = {584--592},
  Url                      = {http://jmlr.org/proceedings/papers/v32/arora14.html},
}
 
@article{AroraLLMR16,
  author    = {Sanjeev Arora and
               Yuanzhi Li and
               Yingyu Liang and
               Tengyu Ma and
               Andrej Risteski},
  title     = {A Latent Variable Model Approach to PMI-based Word Embeddings},
  journal   = {{TACL}},
  volume    = {4},
  pages     = {385--399},
  year      = {2016},
  url       = {https://transacl.org/ojs/index.php/tacl/article/view/742},
} 

@inproceedings{Baker1998,
 author = {Baker, Collin F. and Fillmore, Charles J. and Lowe, John B.},
 title = {The Berkeley FrameNet Project},
 booktitle = {ACL '98},
 year = {1998},
 location = {Montreal, Quebec, Canada},
 pages = {86--90},
 numpages = {5},
 url = {http://dx.doi.org/10.3115/980845.980860},
 doi = {10.3115/980845.980860},
 publisher = {ACL},
 address = {Stroudsburg, PA, USA},
}

@InProceedings{baroni-dinu-kruszewski2014,
  Title                    = {Don't count, predict! A systematic comparison of context-counting vs. context-predicting semantic vectors},
  Author                   = {Baroni, Marco and Dinu, Georgiana and Kruszewski, Germ\'{a}n},
  Booktitle                = {ACL '14},
  Year                     = {2014},
  Address                  = {Baltimore, Maryland},
  Month                    = {June},
  Pages                    = {238--247},
  Publisher                = {Association for Computational Linguistics},
  Url                      = {http://www.aclweb.org/anthology/P/P14/P14-1023}
}

@InProceedings{baroni-lenci-Cognitive-2007,
  Title                    = {{ISA} meets {L}ara: An incremental word space model for cognitively plausible simulations of semantic learning},
  Author                   = {Baroni, Marco and Lenci, Alessandro and Onnis, Luca},
  Booktitle                = {Proceedings of the Workshop on Cognitive Aspects of Computational Language Acquisition},
  Year                     = {2007},
  Address                  = {Prague, Czech Republic},
  Month                    = {June},
  Pages                    = {49--56},
  Publisher                = {Association for Computational Linguistics},
  Url                      = {http://www.aclweb.org/anthology/W/W07/W07-0607}
} 

@InProceedings{Bingham2001RPD,
  Title                    = {Random projection in dimensionality reduction: applications to image and text data},
  Author                   = {Bingham, Ella and Mannila, Heikki},
  Year                     = {2001},
  Address                  = {New York, NY, USA},
  Pages                    = {245--250},
  Publisher                = {ACM},
  Booktitle                   = {KDD '01},
  Acmid                    = {502546},
  Doi                      = {10.1145/502512.502546},
  ISBN                     = {1-58113-391-X},
  Keywords                 = {dimensionality reduction, high-dimensional data, image data, random projection, text document data},
  Location                 = {San Francisco, California},
  Numpages                 = {6},
  Url                      = {http://doi.acm.org/10.1145/502512.502546}
}

@InProceedings{Bouma2009,
  Title                    = {Normalized (Pointwise) Mutual Information in Collocation Extraction},
  Author                   = {Bouma, Gerlof},
  Booktitle                = {Proceedings of the Biennial GSCL Conference},
  Year                     = {2009},
  Journal                  = {Proceedings of the Biennial GSCL Conference}
}

@Article{Bruni2014,
  Title                    = {Multimodal Distributional Semantics},
  Author                   = {Bruni, Elia and Tran, Nam Khanh and Baroni, Marco},
  Journal                  = {J. Artif. Int. Res.},
  Year                     = {2014},
  Month                    = jan,
  Number                   = {1},
  Pages                    = {1--47},
  Volume                   = {49},
  Acmid                    = {2655714},
  Address                  = {USA},
  ISSN                     = {1076-9757},
  Issue_date               = {January 2014},
  Numpages                 = {47},
  Publisher                = {AI Access Foundation},
}

@Article{Bullinaria2012,
author={Bullinaria, John A.
and Levy, Joseph P.},
title={Extracting semantic representations from word co-occurrence statistics: stop-lists, stemming, and SVD},
journal={Behavior Research Methods},
year={2012},
volume={44},
number={3},
pages={890--907},
issn={1554-3528},
doi={10.3758/s13428-011-0183-8},
url={http://dx.doi.org/10.3758/s13428-011-0183-8}
} 

@Article{Bullinaria2012fr,
  author =    {Bullinaria, John A. and Levy, Joseph P.},
  title =     {Extracting semantic representations from word co-occurrence statistics: stop-lists, stemming, and SVD},
  journal =   {Behavior Research Methods},
  year =      {2012},
  volume =    {44},
  number =    {3},
  pages =     {890-907},
  doi =       {10.3758/s13428-011-0183-8},
  keywords =  {Semantic representation; Corpus statistics; SVD},
  language =  {English},
  publisher = {Springer-Verlag},
  url =       {http://dx.doi.org/10.3758/s13428-011-0183-8}
}

@book{chen2006correlation,
  title={Correlation: Parametric and Nonparametric Measures},
  author={Chen, Peter Y. and Popovich, Paula M.},
  series={Quantitative Applications in the Social Sciences},
  year={2002},
  publisher={Sage Publications}
}

@InProceedings{chen-demelo2015,
  author =    {Chen, Jiaqiang and de Melo, Gerard},
  title =     {Semantic Information Extraction for Improved Word Embeddings},
  booktitle = {Proceedings of the 1st Workshop on Vector Space Modeling for Natural Language Processing},
  year =      {2015},
  pages =     {168--175},
  address =   {Denver, Colorado},
  month =     {June},
  publisher = {ACL},
  url =       {http://www.aclweb.org/anthology/W15-1523}
}

@Article{Church1990,
  Title                    = {Word Association Norms, Mutual Information, and Lexicography},
  Author                   = {Church, Kenneth Ward and Hanks, Patrick},
  Journal                  = {Comput. Linguist.},
  Year                     = {1990},
  Number                   = {1},
  Pages                    = {22--29},
  Volume                   = {16},
  Acmid                    = {89095},
  Address                  = {Cambridge, MA, USA},
  ISSN                     = {0891-2017},
  Issue_date               = {March 1990},
  Numpages                 = {8},
  Publisher                = {MIT Press},
}

@Article{Cohen2010,
  Title                    = {Reflective Random Indexing and indirect inference: A scalable method for discovery of implicit connections },
  Author                   = {Trevor Cohen and Roger Schvaneveldt and Dominic Widdows},
  Journal                  = {Journal of Biomedical Informatics },
  Year                     = {2010},
  Number                   = {2},
  Pages                    = {240 - 256},
  Volume                   = {43},
  Doi                      = {http://dx.doi.org/10.1016/j.jbi.2009.09.003},
  ISSN                     = {1532-0464},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S1532046409001208}
}


@Article{CohenSchvaneveldtRindflesch2009,
  author =  {Cohen, Trevor and Schvaneveldt, Roger W and Rindflesch, Thomas C},
  title =   {Predication-based Semantic Indexing: Permutations as a Means to Encode Predications in Semantic Space},
  journal = {AMIA Annual Symposium Proceedings},
  year =    {2009},
  pages =   {114--118}
}

@inproceedings{Collados15,
  author = {Camacho-Collados, Jose and Pilehvar, Mohammad Taher and Navigli, Roberto},
  booktitle = {HLT-NAACL '15},
  isbn = {978-1-941643-49-5},
  pages = {567--577},
  publisher = {ACL},
  title = {NASARI: a Novel Approach to a Semantically-Aware Representation of Items.},
  year = 2015
}

@article{Collobert2011,
 author = {Collobert, Ronan and Weston, Jason and Bottou, L{\'e}on and Karlen, Michael and Kavukcuoglu, Koray and Kuksa, Pavel},
 title = {Natural Language Processing (Almost) from Scratch},
 journal = {J. Mach. Learn. Res.},
 issue_date = {2/1/2011},
 volume = {12},
 month = nov,
 year = {2011},
 issn = {1532-4435},
 pages = {2493--2537},
 numpages = {45},
 url = {http://dl.acm.org/citation.cfm?id=1953048.2078186},
 acmid = {2078186},
 publisher = {JMLR.org},
}


@article{Dasgupta2003,
 author = {Dasgupta, Sanjoy and Gupta, Anupam},
 title = {An Elementary Proof of a Theorem of Johnson and Lindenstrauss},
 journal = {Random Struct. Algorithms},
 issue_date = {January 2003},
 volume = {22},
 number = {1},
 year = {2003},
 issn = {1042-9832},
 pages = {60--65},
 numpages = {6},
 url = {http://dx.doi.org/10.1002/rsa.10073},
 doi = {10.1002/rsa.10073},
 acmid = {639795},
 publisher = {John Wiley \& Sons, Inc.},
 address = {New York, NY, USA},
}

@phdthesis{Evert2004,
author = {Evert, Stefan},
title = {{The statistics of word cooccurrences}},
school={University of Stuttgart},
Year = {2004},
}

@PhdThesis{evert2004statistics,
  author = {Stefan Evert},
  title =  {The statistics of word cooccurrences: word pairs and collocations},
  school = {Institut f{\"u}r maschinelle Sprachverarbeitung, Universit{\"a}t Stuttgart},
  year =   {2004}
}

@article{evert2015,
	author = {Lapesa, Gabriella  and Evert, Stefan },
	title = {A Large Scale Evaluation of Distributional Semantic Models: Parameters, Interactions and Model Selection},
	journal = {{TACL}},
	volume = {2},
	year = {2014},
	publisher = {ACL},
	issn = {2307-387X},
	url = {https://tacl2013.cs.columbia.edu/ojs/index.php/tacl/article/view/457},
	pages = {531--545}
}

@InProceedings{faruqui2014,
  author =    {Faruqui, Manaal and Dyer, Chris},
  title =     {Community Evaluation and Exchange of Word Vectors at wordvectors.org},
  booktitle = {ACL '14},
  year =      {2014},
  address =   {Baltimore, USA},
  month =     {June},
  publisher = {ACL}
}

@inproceedings{FaruquiDJDHS15,
  author    = {Manaal Faruqui and
               Jesse Dodge and
               Sujay Kumar Jauhar and
               Chris Dyer and
               Eduard H. Hovy and
               Noah A. Smith},
  title     = {Retrofitting Word Vectors to Semantic Lexicons},
  booktitle = {{NAACL}-{HLT} '15},
  pages     = {1606--1615},
  year      = {2015},
  url       = {http://aclweb.org/anthology/N/N15/N15-1184.pdf},
 } 
@InProceedings{faruquidyer2014,
  author    = {Faruqui, Manaal  and  Dyer, Chris},
  title     = {Community Evaluation and Exchange of Word Vectors at wordvectors.org},
  booktitle = {ACL '14},
  month     = {June},
  year      = {2014},
  address   = {Baltimore, Maryland},
  publisher = {ACL},
  pages     = {19--24},
  url       = {http://www.aclweb.org/anthology/P/P14/P14-5004}
}


@inproceedings{Finkelstein2001,
  added-at = {2007-11-02T23:09:02.000+0100},
  author = {Finkelstein, Lev and Evgenly, Gabrilovich and Yossi, Matias and Ehud, Rivlin and Zach, Solan and Gadi, Wolfman and Eytan, Ruppin},
  biburl = {http://www.bibsonomy.org/bibtex/2e3da5ac5814391f68a05ef5f08246fcf/bsmyth},
  booktitle = {WWW '10},
  description = {all-bibs-cleaned.bib},
  interhash = {9de5458806a6d69d58732ea14286bf50},
  intrahash = {e3da5ac5814391f68a05ef5f08246fcf},
  keywords = {imported},
  timestamp = {2007-11-02T23:09:10.000+0100},
  title = {{Placing search in context: the concept revisited}},
  year = 2001
}

@inproceedings{Fyshe2015compositional,
  title={A compositional and interpretable semantic space},
  author={Fyshe, Alona and Wehbe, Leila and Talukdar, Partha P and Murphy, Brian and Mitchell, Tom M},
  booktitle={NAACL},
  year={2015}
} 


@inproceedings{ganitkevitch2013ppdb, 
  title = {{PPDB}: The Paraphrase Database}, 
  author = {Ganitkevitch, Juri and {Van Durme}, Benjamin and 
    Callison-Burch, Chris}, 
  booktitle = {Proceedings of NAACL-HLT}, 
  pages = {758--764}, 
  month = {June},   year={2013}, 
  address = {Atlanta, Georgia}, 
  publisher = {ACL}, 
  url = {http://cs.jhu.edu/~ccb/publications/ppdb.pdf} 
} 

@inproceedings{Gillenwater2012,
 author = {Gillenwater, Jennifer and Kulesza, Alex and Taskar, Ben},
 title = {Discovering Diverse and Salient Threads in Document Collections},
 booktitle = {EMNLP-CoNLL '12},
 year = {2012},
 location = {Jeju Island, Korea},
 pages = {710--720},
 numpages = {11},
 url = {http://dl.acm.org/citation.cfm?id=2390948.2391026},
 acmid = {2391026},
 publisher = {ACL},
 address = {Stroudsburg, PA, USA},
}

@article{GKGamma,
 ISSN = {01621459},
 URL = {http://www.jstor.org/stable/2281536},
 author = {Leo A. Goodman and William H. Kruskal},
 journal = {Journal of the American Statistical Association},
 number = {268},
 pages = {732--764},
 publisher = {[American Statistical Association, Taylor & Francis, Ltd.]},
 title = {Measures of Association for Cross Classifications},
 volume = {49},
 year = {1954}
}

@InProceedings{glove2014,
  author    = {Pennington, Jeffrey  and  Socher, Richard  and  Manning, Christopher},
  title     = {Glove: Global Vectors for Word Representation},
  booktitle = {EMNLP '14},
  year      = {2014},
  address   = {Doha, Qatar},
  publisher = {ACL},
  pages     = {1532--1543},
  url       = {http://www.aclweb.org/anthology/D14-1162}
}

  
 @inproceedings{Goyal2012,
 author = {Goyal, Amit and Daum{\'e},III, Hal and Guerra, Raul},
 title = {Fast Large-scale Approximate Graph Construction for NLP},
 booktitle = {EMNLP-CoNLL '12},
 year = {2012},
 location = {Jeju Island, Korea},
 pages = {1069--1080},
 numpages = {12},
 url = {http://dl.acm.org/citation.cfm?id=2390948.2391068},
 acmid = {2391068},
 publisher = {ACL},
 address = {Stroudsburg, PA, USA},
}

@InProceedings{Halawi2012,
  author =    {Halawi, Guy and Dror, Gideon and Gabrilovich, Evgeniy and Koren, Yehuda},
  title =     {Large-scale Learning of Word Relatedness with Constraints},
  year =      {2012},
  booktitle =    {KDD '12},
  pages =     {1406--1414},
  address =   {New York, NY, USA},
  publisher = {ACM},
  acmid =     {2339751},
  doi =       {10.1145/2339530.2339751},
  isbn =      {978-1-4503-1462-6},
  keywords =  {semantic similarity, word relatedness},
  location =  {Beijing, China},
  numpages =  {9},
  url =       {http://doi.acm.org/10.1145/2339530.2339751}
}
@article{Harris1954distributional,
  title={Distributional structure},
  author={Harris, Zellig S},
  journal={Word},
  volume={10},
  number={2-3},
  pages={146--162},
  year={1954},
  publisher={Taylor \& Francis}
}

@Article{Hecht-Nielsen1994,
  author =    {Robert Hecht-Nielsen},
  title =     {Context vectors: general purpose approximate meaning representations self-organized from raw data},
  journal =   {Computational Intelligence: Imitating Life},
  year =      {1994},
  pages =     {43-56},
  owner =     {behqas},
  timestamp = {2013.03.11},
  url =       {http://www.library.itcarlow.ie/record=b1009218~S0}
}

@Article{Hill2015,
  author =     {Hill, Felix and Reichart, Roi and Korhonen, Anna},
  title =      {{SimLex}-999: Evaluating Semantic Models with Genuine Similarity Estimation},
  journal =    {Comput. Linguist.},
  year =       {2015},
  volume =     {41},
  number =     {4},
  pages =      {665--695},
  month =      dec,
  acmid =      {2893324},
  address =    {Cambridge, MA, USA},
  doi =        {10.1162/COLI_a_00237},
  issn =       {0891-2017},
  issue_date = {December 2015},
  numpages =   {31},
  publisher =  {MIT Press},
  url =        {http://dx.doi.org/10.1162/COLI_a_00237}
}

@InProceedings{Indyk2000,
  Title                    = {Stable distributions, pseudorandom generators, embeddings and data stream computation},
  Author                   = {Piotr  Indyk},
  Booktitle                = {41st Annual Symposium on Foundations of Computer Science},
  Year                     = {2000},
  Pages                    = {189-197},
  Doi                      = {10.1109/SFCS.2000.892082},
  ISSN                     = {0272-5428},
  Keywords                 = {probability;random number generation;bounded space;data stream computation;dimensionality reduction;embeddings;pseudorandom generators;stable distributions;Counting circuits;Distributed computing;Distributed power generation;Embedded computing;Power generation;Statistics;Tail}
}


@InCollection{johnson84extensionslipschitz,
  Title                    = {Extensions of {L}ipschitz mappings into a {H}ilbert space},
  Author                   = {Johnson, William and Lindenstrauss, Joram},
  Booktitle                = {Conference in modern analysis and probability},
  Publisher                = {AMS},
  Year                     = {1984},
  Pages                    = {189--206},
  Volume                   = {26},
  Citeulike-article-id     = {7030987},
  Doi                      = {http://dx.doi.org/10.1090/conm/026},
  Keywords                 = {hilbert, mappings, spaces},
  Posted-at                = {2010-08-24 14:44:11},
  Url                      = {http://www.ams.org/books/conm/026/}
}

@Article{Jones1987,
  Title                    = {Pictures of relevance: A geometric analysis of similarity measures},
  Author                   = {Jones, William P. and Furnas, George W.},
  Journal                  = {Journal of the American Society for Information Science},
  Year                     = {1987},
  Number                   = {6},
  Pages                    = {420--442},
  Volume                   = {38},
  Doi                      = {10.1002/(SICI)1097-4571(198711)38:6<420::AID-ASI3>3.0.CO;2-S},
  ISSN                     = {1097-4571},
  Publisher                = {Wiley Subscription Services, Inc., A Wiley Company},
  Url                      = {http://dx.doi.org/10.1002/(SICI)1097-4571(198711)38:6<420::AID-ASI3>3.0.CO;2-S}
}

@inproceedings{LiuJWH16,
  author    = {Hong Liu and
               Rongrong Ji and
               Yongjian Wu and
               Gang Hua},
  title     = {Supervised Matrix Factorization for Cross-Modality Hashing},
  booktitle = {Proceedings of the Twenty-Fifth International Joint Conference on
               Artificial Intelligence, {IJCAI} 2016},
  pages     = {1767--1773},
  year      = {2016},
}

@inproceedings{Geva2011TTP,
 author = {Geva, Shlomo and De Vries, Christopher M.},
 title = {TOPSIG: Topology Preserving Document Signatures},
 booktitle = {CIKM '11},
 year = {2011},
 isbn = {978-1-4503-0717-8},
 location = {Glasgow, Scotland, UK},
 pages = {333--338},
 numpages = {6},
 url = {http://doi.acm.org/10.1145/2063576.2063629},
 doi = {10.1145/2063576.2063629},
 acmid = {2063629},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {document clustering, document signatures, quantisation, random indexing, search engines, signature files, topology, vector space IR},
} 

@TechReport{citeulike2706665,
  author =               {Michael},
  title =                {{Fingerprinting by random polynomials}},
  institution =          {Center of Research in Computer Technology},
  year =                 {1981},
  booktitle =            {Technical Report TR-15-81},
  citeulike-article-id = {2706665},
  keywords =             {datadeduplication},
  posted-at =            {2008-04-23 10:25:38},
  school =               {Hardward University}
}

@article{DeerwesterDLFH90,
  author    = {Scott C. Deerwester and
               Susan T. Dumais and
               Thomas K. Landauer and
               George W. Furnas and
               Richard A. Harshman},
  title     = {Indexing by Latent Semantic Analysis},
  journal   = {{JASIS}},
  volume    = {41},
  number    = {6},
  pages     = {391--407},
  year      = {1990},
  doi       = {10.1002/(SICI)1097-4571(199009)41:6<391::AID-ASI1>3.0.CO;2-9},
 
}

@InProceedings{qzadehhandschuh2014EMNLP2014,
  author    = {Q. Zadeh, Behrang  and  Handschuh, Siegfried},
  title     = {Random Manhattan Integer Indexing: Incremental L1 Normed Vector Space Construction},
  booktitle = {EMNLP},
  year      = {2014},
  address   = {Doha, Qatar},
  publisher = {ACL},
  pages     = {1713--1723},
  url       = {http://www.aclweb.org/anthology/D14-1178}
}

@inproceedings{qasemiZadeh15ri,
  author    = {Behrang QasemiZadeh},
  title     = {Random Indexing Revisited},
  booktitle = {NLDB},
  pages     = {437--442},
  year      = {2015},
  url       = {http://dx.doi.org/10.1007/978-3-319-19581-0_43},
  doi       = {10.1007/978-3-319-19581-0_43},
}

@inproceedings{kanerva00random,
  author = {Kanerva, P. and Kristofersson, J. and Holst, A.},
  booktitle = {Proceedings of the 22nd Annual Conference of the                   Cognitive Science Society},
  title = {Random Indexing of Text Samples for Latent Semantic Analysis},
  volume = 1036,
  year = 2000
}
@INPROCEEDINGS{kaski1998, 
author={S. Kaski}, 
booktitle={IEEE International Joint Conference on Neural Networks Proceedings}, 
title={Dimensionality reduction by random mapping: fast similarity computation for clustering}, 
year={1998}, 
volume={1}, 
pages={413-418 vol.1}, 
keywords={data analysis;document image processing;pattern matching;self-organising feature maps;WEBSOM method;clustering;data analysis;data vectors;dimensionality reduction;document image processing;pattern recognition;random mapping method;self-organizing map;similarity computation;Clustering algorithms;Computer networks;Data analysis;Feature extraction;Multidimensional systems;Neural networks;Organizing;Pattern recognition;Space technology;Vectors}, 
doi={10.1109/IJCNN.1998.682302}, 
ISSN={1098-7576}, 
month={May}
}

@inproceedings{Bingham2001,
 author = {Bingham, Ella and Mannila, Heikki},
 title = {Random Projection in Dimensionality Reduction: Applications to Image and Text Data},
 booktitle = {Proceedings of the Seventh ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
 series = {KDD '01},
 year = {2001},
 isbn = {1-58113-391-X},
 location = {San Francisco, California},
 pages = {245--250},
 numpages = {6},
 url = {http://doi.acm.org/10.1145/502512.502546},
 doi = {10.1145/502512.502546},
 acmid = {502546},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {dimensionality reduction, high-dimensional data, image data, random projection, text document data},
}

@inproceedings{Dalvi2013,
 author = {Dalvi, Nilesh and Rastogi, Vibhor and Dasgupta, Anirban and Das Sarma, Anish and Sarlos, Tamas},
 title = {Optimal Hashing Schemes for Entity Matching},
 booktitle = {WWW '13},
 year = {2013},
 isbn = {978-1-4503-2035-1},
 location = {Rio de Janeiro, Brazil},
 pages = {295--306},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/2488388.2488415},
 doi = {10.1145/2488388.2488415},
 acmid = {2488415},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {blocking, entity matching, hashing},
} 

@inproceedings{Wang2015,
 author = {Wang, Di and Gao, Xinbo and Wang, Xiumei and He, Lihuo},
 title = {Semantic Topic Multimodal Hashing for Cross-media Retrieval},
 booktitle = {IJCAI'15},
 year = {2015},
 isbn = {978-1-57735-738-4},
 location = {Buenos Aires, Argentina},
 pages = {3890--3896},
 numpages = {7},
 url = {http://dl.acm.org/citation.cfm?id=2832747.2832791},
 acmid = {2832791},
 publisher = {AAAI Press},
}

@inproceedings{YangLC16,
  author    = {Dingqi Yang and
               Bin Li and
               Philippe Cudr{\'{e}}{-}Mauroux},
  title     = {POISketch: Semantic Place Labeling over User Activity Streams},
  booktitle = {Proceedings of the Twenty-Fifth International Joint Conference on
               Artificial Intelligence, {IJCAI} 2016},
  pages     = {2697--2703},
  year      = {2016},
}

@inproceedings{Manku2007,
 author = {Manku, Gurmeet Singh and Jain, Arvind and Das Sarma, Anish},
 title = {Detecting Near-duplicates for Web Crawling},
 booktitle = {WWW '07},
 year = {2007},
 isbn = {978-1-59593-654-7},
 location = {Banff, Alberta, Canada},
 pages = {141--150},
 numpages = {10},
 doi = {10.1145/1242572.1242592},
 acmid = {1242592},
 publisher = {ACM},
 address = {New York, NY, USA},
} 


@InBook{JurafskyMartin2015,
  Title                    = {Speech and Language Processing},
  Author                   = {Daniel Jurafsky and James H. Martin},
  Chapter                  = {Chapter 19: Vector Semantics},
  publisher  = {Prentice Hall},
  Year                     = {2015},
  Edition                  = {3rd},
  Note                     = {Draft of August 24, 2015}
}

@InProceedings{Kanerva00randomindexing,
  Title                    = {Random Indexing of Text Samples for Latent Semantic Analysis},
  Author                   = {Pentti Kanerva and Jan Kristoferson and Anders Holst},
  Booktitle                = {Proceedings of the 22nd Annual Conference of the CogSci},
  Year                     = {2000},
  Pages                    = {103--6},
  Publisher                = {Erlbaum},
  Url                      = {http://www.rni.org/kanerva/cogsci2k-poster.txt}
}

@Article{Karp1991165,
  Title                    = {An introduction to randomized algorithms },
  Author                   = {Richard M. Karp},
  Journal                  = {Discrete Applied Mathematics },
  Year                     = {1991},
  Number                   = {1–3},
  Pages                    = {165 - 201},
  Volume                   = {34},
  Doi                      = {http://dx.doi.org/10.1016/0166-218X(91)90086-C},
  ISSN                     = {0166-218X},
  Url                      = {http://www.sciencedirect.com/science/article/pii/0166218X9190086C}
}

@InProceedings{Kaski1998RT,
  author =    {Samuel Kaski},
  title =     {Dimensionality reduction by random mapping: fast similarity computation for clustering},
  booktitle = {The 1998 IEEE IJCNN},
  year =      {1998},
  volume =    {1},
  pages =     {413-418},
  doi =       {10.1109/IJCNN.1998.682302},
  issn =      {1098-7576},
  url =       {http://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=682302&isnumber=15009}
}

@Article{KENDALL01061938,
  Title                    = {A New Measure of Rank Correlation},
  Author                   = {Maurice G. Kendall},
  Journal                  = {Biometrika},
  Year                     = {1938},
  Number                   = {1-2},
  Pages                    = {81-93},
  Volume                   = {30},
  Doi                      = {10.1093/biomet/30.1-2.81},
  Eprint                   = {http://biomet.oxfordjournals.org/content/30/1-2/81.full.pdf+html},
  Url                      = {http://biomet.oxfordjournals.org/content/30/1-2/81.short}
}

@Book{Kendall1948,
  Title                    = {Rank correlation methods},
  Author                   = {Maurice Kendall},
  Publisher                = {Oxford University Press},
  Year                     = {1948}
}

@InProceedings{kiela-clark2014CVSC,
  Title                    = {A Systematic Study of Semantic Vector Space Model Parameters},
  Author                   = {Kiela, Douwe and Clark, Stephen},
  Booktitle                = {Proceedings of the 2nd Workshop on Continuous Vector Space Models and their Compositionality (CVSC)},
  Year                     = {2014},
  Address                  = {Gothenburg, Sweden},
  Month                    = {April},
  Pages                    = {21--30},
  Publisher                = {ACL},
  Url                      = {http://www.aclweb.org/anthology/W14-1503}
}

@Article{Knight66,
  Title                    = {A Computer Method for Calculating Kendall's Tau with Ungrouped Data},
  Author                   = {William R. Knight},
  Journal                  = {Journal of the American Statistical Association},
  Year                     = {1966},
  Number                   = {314},
  Pages                    = {436-439},
  Volume                   = {61},
  Abstract                 = {Adapting the usual manual methods of computing Kendall's tau to automatic computation result in a running time of order N<sup>2</sup>. A method is described with running time of order N log N.},
  ISSN                     = {01621459},
  Publisher                = {[American Statistical Association, Taylor \& Francis, Ltd.]},
  Url                      = {http://www.jstor.org/stable/2282833}
}

@Article{landauer97solution,
  author =               {Landauer, T. and Dumais, S.},
  title =                {{A Solution to Plato's Problem: The Latent Semantic Analysis Theory of Acquisition, Induction and Representation of Knowledge}},
  journal =              {Psychological Review},
  year =                 {1997},
  volume =               {104},
  pages =                {411--240},
 }
 
@inproceedings{Levy2014linguistic,
  title={Linguistic Regularities in Sparse and Explicit Word Representations},
  author={Levy, Omer and Goldberg, Yoav and Ramat-Gan, Israel},
  booktitle={CoNLL},
  pages={171--180},
  year={2014}
}



@inproceedings{Levy2014neural,
 Title                    = {Neural Word Embedding as Implicit Matrix Factorization},
  Author                   = {Levy, Omer and Goldberg, Yoav},
  Booktitle                = {NIPS 27},
  Year                     = {2014},
  Pages                    = {2177--2185},
  Url                      = {http://papers.nips.cc/paper/5477-neural-word-embedding-as-implicit-matrix-factorization.pdf}
}

@article{Levy2015improving,
  title={Improving distributional similarity with lessons learned from word embeddings},
  author={Levy, Omer and Goldberg, Yoav and Dagan, Ido},
  journal={{TACL}},
  volume={3},
  pages={211--225},
  year={2015}
}

@InProceedings{Li2006VSR,
  Title                    = {Very Sparse Random Projections},
  Author                   = {Li, Ping and Hastie, Trevor J. and Church, Kenneth W.},
  Year                     = {2006},
  Address                  = {New York, NY, USA},
  Pages                    = {287--296},
  Publisher                = {ACM},
  Booktitle                   = {KDD '06},
  Acmid                    = {1150436},
  Doi                      = {10.1145/1150402.1150436},
  ISBN                     = {1-59593-339-5},
  Keywords                 = {random projections, rates of convergence, sampling},
  Location                 = {Philadelphia, PA, USA},
  Numpages                 = {10},
  Url                      = {http://doi.acm.org/10.1145/1150402.1150436}
}

@Inbook{Li2007,
author={Li, Ping
and Hastie, Trevor J.
and Church, Kenneth W.},
chapter="Nonlinear Estimators and Tail Bounds for Dimension Reduction in l1 Using Cauchy Random Projections",
title="Learning Theory: 20th Annual Conference on Learning Theory, COLT 2007, San Diego, CA, USA; June 13-15, 2007. Proceedings",
year="2007",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="514--529",
isbn="978-3-540-72927-3",
doi="10.1007/978-3-540-72927-3_37",
url="http://dx.doi.org/10.1007/978-3-540-72927-3_37"
}

@inproceedings{Li2015word,
  title={Word embedding revisited: A new representation learning and explicit matrix factorization perspective},
  author={Li, Yitan and Xu, Linli and Tian, Fei and Jiang, Liang and Zhong, Xiaowei and Chen, Enhong},
  booktitle={IJCAI '15},
  pages={3650--3656},
  year={2015}
}

@article{bojanowski2017enriching,
  title={Enriching Word Vectors with Subword Information},
  author={Bojanowski, Piotr and Grave, Edouard and Joulin, Armand and Mikolov, Tomas},
  journal={Transactions of the Association for Computational Linguistics},
  volume={5},
  year={2017},
  issn={2307-387X},
  pages={135--146}
}

@Article{MC30,
  author =  {George A. Miller and Walter G. Charles},
  title =   {Contextual correlates of semantic similarity},
  journal = {Language and Cognitive Processes},
  year =    {1991},
  volume =  {6},
  number =  {1},
  pages =   {1-28},
  doi =     {10.1080/01690969108406936},
  eprint =  {http://dx.doi.org/10.1080/01690969108406936},
  url =     {http://dx.doi.org/10.1080/01690969108406936}
}

@article{mikoAna,
  author    = {Tomas Mikolov and
               Kai Chen and
               Greg Corrado and
               Jeffrey Dean},
  title     = {Efficient Estimation of Word Representations in Vector Space},
  journal   = {CoRR},
  volume    = {abs/1301.3781},
  year      = {2013},
  url       = {http://arxiv.org/abs/1301.3781},
}

@inproceedings{Mikolov2013,
  Title                    = {Distributed Representations of Words and Phrases and their Compositionality},
  Author                   = {Mikolov, Tomas and Sutskever, Ilya and Chen, Kai and Corrado, Greg S and Dean, Jeff},
  booktitle                = {NIPS 26},
  Year                     = {2013},
Pages                    = {3111--3119},
  Url                      = {http://papers.nips.cc/paper/5021-distributed-representations-of-words-and-phrases-and-their-compositionality.pdf}
} 

@article{Miller1995,
 author = {Miller, George A.},
 title = {WordNet: A Lexical Database for English},
 journal = {Commun. ACM},
 issue_date = {Nov. 1995},
 volume = {38},
 number = {11},
 month = nov,
 year = {1995},
 issn = {0001-0782},
 pages = {39--41},
 numpages = {3},
 url = {http://doi.acm.org/10.1145/219717.219748},
 doi = {10.1145/219717.219748},
 acmid = {219748},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@Book{MinskyPapert1969,
  Title                    = {Perceptrons: An Introduction to Computational Geometry},
  Author                   = {Marvin Lee Minsky and Seymour Papert},
  Publisher                = {MIT Press},
  Year                     = {1969}
} 

@InProceedings{petrov2008,
  author    = {Petrov, Slav  and  Haghighi, Aria  and  Klein, Dan},
  title     = {Coarse-to-Fine Syntactic Machine Translation using Language Projections},
  booktitle = {EMNLP '8},
  year      = {2008},
  address   = {Honolulu, Hawaii},
  publisher = {ACL},
  pages     = {108--116},
  url       = {http://www.aclweb.org/anthology/D08-1012}
}



@InProceedings{QasemiZadeh2015,
  author =    {QasemiZadeh, Behrang},
  title =     {{NLDB}},
  booktitle = {NLDB},
  year =      {2015},
  pages =     {437--442},
  publisher = {Springer},
  chapter =   {Random Indexing Revisited},
  doi =       {10.1007/978-3-319-19581-0_43},
  isbn =      {978-3-319-19581-0},
  url =       {http://dx.doi.org/10.1007/978-3-319-19581-0_43}
}

@InProceedings{Radinsky2011,
  author =    {Radinsky, Kira and Agichtein, Eugene and Gabrilovich, Evgeniy and Markovitch, Shaul},
  title =     {A Word at a Time: Computing Word Relatedness Using Temporal Semantic Analysis},
  year =      {2011},
  booktitle =    {WWW '11},
  pages =     {337--346},
  address =   {New York, NY, USA},
  publisher = {ACM},
  acmid =     {1963455},
  doi =       {10.1145/1963405.1963455},
  isbn =      {978-1-4503-0632-4},
  keywords =  {semantic analysis, semantic similarity, temporal dynamics, temporal semantics, word relatedness},
  location =  {Hyderabad, India},
  numpages =  {10},
  url =       {http://doi.acm.org/10.1145/1963405.1963455}
}

@Article{RG1965,
  author =     {Rubenstein, Herbert and Goodenough, John B.},
  title =      {Contextual Correlates of Synonymy},
  journal =    {Commun. ACM},
  year =       {1965},
  volume =     {8},
  number =     {10},
  pages =      {627--633},
  acmid =      {365657},
  address =    {New York, NY, USA},
  doi =        {10.1145/365628.365657},
  issn =       {0001-0782},
  issue_date = {Oct. 1965},
  numpages =   {7},
  publisher =  {ACM},
  url =        {http://doi.acm.org/10.1145/365628.365657}
}

@article{Rubenstein1965,
 author = {Rubenstein, Herbert and Goodenough, John B.},
 title = {Contextual Correlates of Synonymy},
 journal = {Commun. ACM},
 issue_date = {Oct. 1965},
 volume = {8},
 number = {10},
 month = oct,
 year = {1965},
 issn = {0001-0782},
 pages = {627--633},
 numpages = {7},
 url = {http://doi.acm.org/10.1145/365628.365657},
 doi = {10.1145/365628.365657},
 acmid = {365657},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@InProceedings{rw2013,
  author =    {Luong, Thang and Socher, Richard and Manning, Christopher D},
  title =     {Better Word Representations with Recursive Neural Networks for Morphology.},
  booktitle = {CoNLL},
  year =      {2013},
  pages =     {104--113},
  publisher = {ACL}
}

@InProceedings{sahl2008,
  Title                    = {Permutations as a means to encode order in word space},
  Author                   = {Sahlgren, Magnus and Holst, Anders and Kanerva, Pentti},
  Booktitle                = {CogSci},
  Year                     = {2008},
}

@InCollection{Sahlgren2008,
  author =               {Sahlgren, Magnus and Holst, Anders and Kanerva, Pentti},
  title =                {{Permutations as a means to encode order in word space}},
  booktitle =            {Proceedings of the 30th Annual Conference of the Cognitive Science Society},
  publisher =            {Cognitive Science Society},
  year =                 {2008},
pages =                {1300--1305},
  address =              {Austin, TX},
  citeulike-article-id = {3132971},
  citeulike-linkout-0 =  {http://www.sics.se/\~{}mange/papers/permutationsCogSci08.pdf},
  keywords =             {distributional-similarity},
  posted-at =            {2008-08-18 16:01:17},
  url =                  {http://www.sics.se/\~{}mange/papers/permutationsCogSci08.pdf}
}

@InProceedings{SchaeferBildhauer2012,
  author =    {Roland Schafer and Felix Bildhauer},
  title =     {Building Large Corpora from the Web Using a New Efficient Tool Chain},
  booktitle = {LREC'12},
  year =      {2012},
  pages =     {486--493}
}

@techreport{browncorpus,
  author = {Francis, W. Nelson and Kucera, Henry},
  institution = {Brown University},
  title = {Brown Corpus Manual},
  url = {http://icame.uib.no/brown/bcm.html},
  year = 1979
}


 @InProceedings{schnabel2015,
  author    = {Schnabel, Tobias  and  Labutov, Igor  and  Mimno, David  and  Joachims, Thorsten},
  title     = {Evaluation methods for unsupervised word embeddings},
  booktitle = {EMNLP},
  month     = {September},
  year      = {2015},
  address   = {Lisbon, Portugal},
  publisher = {ACL},
  pages     = {298--307},
  url       = {http://aclweb.org/anthology/D15-1036}
}

@book{sinclair2004trust,
  title={Trust the Text: Language, Corpus and Discourse},
  author={John Sinclair},
  isbn={9781134369928},
  year={2004},
  publisher={Taylor \& Francis}
}

@inproceedings{Stein2007,
 author = {Stein, Benno},
 title = {Principles of Hash-based Text Retrieval},
 booktitle = {SIGIR '07},
 year = {2007},
 isbn = {978-1-59593-597-7},
 location = {Amsterdam, The Netherlands},
 pages = {527--534},
 numpages = {8},
 url = {http://doi.acm.org/10.1145/1277741.1277832},
 doi = {10.1145/1277741.1277832},
 acmid = {1277832},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@inproceedings{Stratos2015model,
  title={Model-based word embeddings from decompositions of count matrices},
  author={Stratos, Karl and Collins, Michael and Hsu, Daniel},
  booktitle={ACL},
  year={2015}
}



@InProceedings{tsvetkov2015EMNLP,
  Title                    = {Evaluation of Word Vector Representations by Subspace Alignment},
  Author                   = {Tsvetkov, Yulia and Faruqui, Manaal and Ling, Wang and Lample, Guillaume and Dyer, Chris},
  Booktitle                = {EMNLP '15},
  Year                     = {2015},
  Address                  = {Lisbon, Portugal},
  Month                    = {September},
  Pages                    = {2049--2054},
  Publisher                = {ACL},
}

@InProceedings{Turney2001,
  Title                    = {Mining the Web for Synonyms: {PMI-IR} Versus {LSA} on {TOEFL}},
  Author                   = {Turney, Peter D.},
  Year                     = {2001},
  Address                  = {London, UK, UK},
  Pages                    = {491--502},
  Publisher                = {Springer-Verlag},
  Booktitle                   = {EMCL '01},
  ISBN                     = {3-540-42536-5},
 
}

@Article{Turney2008LRM,
  Title                    = {The Latent Relation Mapping Engine: Algorithm and Experiments},
  Author                   = {Turney, Peter D.},
  Journal                  = {J. Artif. Int. Res.},
  Year                     = {2008},
  Month                    = dec,
  Number                   = {1},
  Pages                    = {615--655},
  Volume                   = {33},
  Acmid                    = {1622715},
  Address                  = {USA},
  ISSN                     = {1076-9757},
  Issue_date               = {September 2008},
  Numpages                 = {41},
  Publisher                = {AI Access Foundation},
  Url                      = {http://dl.acm.org/citation.cfm?id=1622698.1622715}
}

@Article{Turney2010,
  Title                    = {From Frequency to Meaning: Vector Space Models of Semantics},
  Author                   = {Turney, Peter D. and Pantel, Patrick},
  Journal                  = {J. Artif. Int. Res.},
  Year                     = {2010},
  Month                    = jan,
  Number                   = {1},
  Pages                    = {141--188},
  Volume                   = {37},
  Acmid                    = {1861756},
  Address                  = {USA},
  ISSN                     = {1076-9757},
  Issue_date               = {January 2010},
  Numpages                 = {48},
  Publisher                = {AI Access Foundation},
  Url                      = {http://dl.acm.org/citation.cfm?id=1861751.1861756}
}

@inproceedings{Udupa2010,
 author = {Udupa, Raghavendra and Kumar, Shaishav},
 title = {Hashing-based Approaches to Spelling Correction of Personal Names},
 booktitle = {EMNLP '10},
 year = {2010},
 location = {Cambridge, Massachusetts},
 pages = {1256--1265},
 numpages = {10},
 url = {http://dl.acm.org/citation.cfm?id=1870658.1870780},
 acmid = {1870780},
 publisher = {ACL},
 address = {Stroudsburg, PA, USA},
}

@Article{Wacku2009,
  Title                    = {The WaCky wide web: a collection of very large linguistically processed web-crawled corpora},
  Author                   = {Baroni, Marco and Bernardini, Silvia and Ferraresi, Adriano and Zanchetta, Eros},
  Journal                  = {LRE},
  Year                     = {2009},
  Number                   = {3},
  Pages                    = {209-226},
  Volume                   = {43},
  Doi                      = {10.1007/s10579-009-9081-4},
  ISSN                     = {1574-020X},
  Keywords                 = {Annotated corpora; Corpus construction; General-purpose linguistic resources; English; German; Italian; Web as corpus; WaCky!},
  Language                 = {English},
  Publisher                = {Springer Netherlands},
  Url                      = {http://dx.doi.org/10.1007/s10579-009-9081-4}
}

@InProceedings{Yang06,
  author =    {Dongqiang Yang and David M. W. Powers},
  title =     {Verb Similarity on the Taxonomy of Wordnet},
  booktitle = {GWC-06},
  year =      {2006},
  address =   {Jeju Island, Korea}
}

@inproceedings{YinS16,
  author    = {Wenpeng Yin and
               Hinrich Sch{\"{u}}tze},
  title     = {Learning Word Meta-Embeddings},
  booktitle = {ACL},
  year      = {2016},
}

@InProceedings{ZadehH14,
  Title                    = {Random Manhattan Integer Indexing: Incremental {L1} Normed Vector Space Construction},
  Author                   = {Behrang Q. Zadeh and Siegfried Handschuh},
  Booktitle                = {EMNLP},
  Year                     = {2014},
  Pages                    = {1713--1723},
  Url                      = {http://aclweb.org/anthology/D/D14/D14-1178.pdf}
}


@inproceedings{le2014distributed,
  title={Distributed Representations of Sentences and Documents.},
  author={Le, Quoc V and Mikolov, Tomas},
  booktitle={ICML},
  volume={14},
  pages={1188--1196},
  year={2014}
}

@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997},
  publisher={MIT Press}
}


@inproceedings{Charikar:2002:SET,
 author = {Charikar, Moses S.},
 title = {Similarity Estimation Techniques from Rounding Algorithms},
 booktitle = {Proceedings of the Thiry-fourth Annual ACM Symposium on Theory of Computing},
 series = {STOC '02},
 year = {2002},
 isbn = {1-58113-495-9},
 location = {Montreal, Quebec, Canada},
 pages = {380--388},
 numpages = {9},
 url = {http://doi.acm.org/10.1145/509907.509965},
 doi = {10.1145/509907.509965},
 acmid = {509965},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@InProceedings{vandurme-lall:2011:ACL-HLT2011,
  author    = {Van Durme, Benjamin  and  Lall, Ashwin},
  title     = {Efficient Online Locality Sensitive Hashing via Reservoir Counting},
  booktitle = {Proceedings of the 49th Annual Meeting of the Association for Computational Linguistics: Human Language Technologies},
  month     = {June},
  year      = {2011},
  address   = {Portland, Oregon, USA},
  publisher = {Association for Computational Linguistics},
  pages     = {18--23},
  url       = {http://www.aclweb.org/anthology/P11-2004}
}

@inproceedings{Indyk1998:ANN,
 author = {Indyk, Piotr and Motwani, Rajeev},
 title = {Approximate Nearest Neighbors: Towards Removing the Curse of Dimensionality},
 booktitle = {Proceedings of the Thirtieth Annual ACM Symposium on Theory of Computing},
 series = {STOC '98},
 year = {1998},
 isbn = {0-89791-962-9},
 location = {Dallas, Texas, USA},
 pages = {604--613},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/276698.276876},
 doi = {10.1145/276698.276876},
 acmid = {276876},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@InProceedings{vandurme-lall:2010:Short,
  author    = {Van Durme, Benjamin  and  Lall, Ashwin},
  title     = {Online Generation of Locality Sensitive Hash Signatures},
  booktitle = {Proceedings of the ACL 2010 Conference Short Papers},
  month     = {July},
  year      = {2010},
  address   = {Uppsala, Sweden},
  publisher = {Association for Computational Linguistics},
  pages     = {231--235},
  url       = {http://www.aclweb.org/anthology/P10-2043}
}

@InProceedings{ravichandran-pantel-hovy:2005:ACL,
  author    = {Ravichandran, Deepak  and  Pantel, Patrick  and  Hovy, Eduard},
  title     = {Randomized Algorithms and {NLP}: Using Locality Sensitive Hash Functions for High Speed Noun Clustering},
  booktitle = {Proceedings of the 43rd Annual Meeting of the Association for Computational Linguistics (ACL'05)},
  month     = {June},
  year      = {2005},
  address   = {Ann Arbor, Michigan},
  publisher = {Association for Computational Linguistics},
  pages     = {622--629},
  url       = {http://www.aclweb.org/anthology/P05-1077},
  doi       = {10.3115/1219840.1219917}
}


@InProceedings{rastogi-vandurme-arora:2015:NAACL-HLT,
  author    = {Rastogi, Pushpendre  and  Van Durme, Benjamin  and  Arora, Raman},
  title     = {Multiview {LSA}: Representation Learning via Generalized {CCA}},
  booktitle = {Proceedings of the 2015 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
  month     = {May--June},
  year      = {2015},
  address   = {Denver, Colorado},
  publisher = {Association for Computational Linguistics},
  pages     = {556--566},
  url       = {http://www.aclweb.org/anthology/N15-1058}
}


@inproceedings{Xu:2015:CNN:2832415.2832440,
 author = {Xu, Jiaming and Wang, Peng and Tian, Guanhua and Xu, Bo and Zhao, Jun and Wang, Fangyuan and Hao, Hongwei},
 title = {Convolutional Neural Networks for Text Hashing},
 booktitle = {Proceedings of the 24th International Conference on Artificial Intelligence},
 series = {IJCAI'15},
 year = {2015},
 isbn = {978-1-57735-738-4},
 location = {Buenos Aires, Argentina},
 pages = {1369--1375},
 numpages = {7},
 url = {http://dl.acm.org/citation.cfm?id=2832415.2832440},
 acmid = {2832440},
 publisher = {AAAI Press},
} 

@inproceedings{ChappellG15,
  author    = {Timothy Chappell and
               Shlomo Geva},
  title     = {TopSig: {A} Scalable System for Hashing and Retrieving Document Signatures},
  booktitle = {Information Retrieval Technology - 11th Asia Information Retrieval
               Societies Conference, {AIRS} 2015, Brisbane, QLD, Australia, December
               2-4, 2015. Proceedings},
  pages     = {447--452},
  year      = {2015},
  url       = {https://doi.org/10.1007/978-3-319-28940-3_40},
  doi       = {10.1007/978-3-319-28940-3_40},
}

@inproceedings{Shrivastava2015AMH,
 author = {Shrivastava, Anshumali and Li, Ping},
 title = {Asymmetric Minwise Hashing for Indexing Binary Inner Products and Set Containment},
 booktitle = {Proceedings of the 24th International Conference on World Wide Web},
 series = {WWW '15},
 year = {2015},
 isbn = {978-1-4503-3469-3},
 location = {Florence, Italy},
 pages = {981--991},
 numpages = {11},
 url = {https://doi.org/10.1145/2736277.2741285},
 doi = {10.1145/2736277.2741285},
 acmid = {2741285},
 publisher = {International World Wide Web Conferences Steering Committee},
 address = {Republic and Canton of Geneva, Switzerland},
 keywords = {asymmetric minwise hashing, indexing, maximum inner product search},
} 

@InProceedings{polyglot:2013:ACL-CoNLL,
  author    = {Al-Rfou, Rami  and  Perozzi, Bryan  and  Skiena, Steven},
  title     = {Polyglot: Distributed Word Representations for Multilingual NLP},
  booktitle = {Proceedings of the Seventeenth Conference on Computational Natural Language Learning},
  month     = {August},
  year      = {2013},
  address   = {Sofia, Bulgaria},
  publisher = {Association for Computational Linguistics},
  pages     = {183--192}, 
  url       = {http://www.aclweb.org/anthology/W13-3520}
}



@InProceedings{kim:2014:EMNLP2014,
  author    = {Kim, Yoon},
  title     = {Convolutional Neural Networks for Sentence Classification},
  booktitle = {Proceedings of the 2014 Conference on Empirical Methods in Natural Language Processing (EMNLP)},
  month     = {October},
  year      = {2014},
  address   = {Doha, Qatar},
  publisher = {Association for Computational Linguistics},
  pages     = {1746--1751},
  url       = {http://www.aclweb.org/anthology/D14-1181}
}


@InProceedings{maas-EtAl:2011:ACL-HLT2011,
  author    = {Maas, Andrew L.  and  Daly, Raymond E.  and  Pham, Peter T.  and  Huang, Dan  and  Ng, Andrew Y.  and  Potts, Christopher},
  title     = {Learning Word Vectors for Sentiment Analysis},
  booktitle = {Proceedings of the 49th Annual Meeting of the Association for Computational Linguistics: Human Language Technologies},
  month     = {June},
  year      = {2011},
  address   = {Portland, Oregon, USA},
  publisher = {Association for Computational Linguistics},
  pages     = {142--150},
  url       = {http://www.aclweb.org/anthology/P11-1015}
}



==> results/classic.tex <==
run:
Dim is 5463172
                           RW      2951
                        V-143       117
                           EN       916
                     MTURK287       499
                     MTURK771      1113
                         RG65        48
                          WS0       437
                          WSS       277
                         MC30        39
                          MEN       751
                          WSR       346
                           YP       147
                       Sim999      1028
count	         RW      V-143         EN   MTURK287   MTURK771       RG65        WS0        WSS       MC30        MEN        WSR         YP     Sim999
	7.40611.3066.85417.23115.54242.77128.10040.41149.22924.80816.95713.33012.365	SimCosine	WNone
&   0.07&   0.11&   0.07&   0.17&   0.16&   0.43&   0.28&   0.40&   0.49&   0.25&   0.17&   0.13&   0.12
	31.73742.36955.69452.56756.13479.52650.09054.61279.93268.43261.51943.06628.586	SimCosine	WPPMI
&   0.32&   0.42&   0.56&   0.53&   0.56&   0.80&   0.50&   0.55&   0.80&   0.68&   0.62&   0.43&   0.29
BUILD SUCCESSFUL (total time: 61 minutes 30 seconds)


==> weightings/combinedweigh.tex <==
\pgfplotstableread{
nz  dim ctxLeft ctxRight    max min ave
2	300	-2	2	0.8625	0.7375	0.79625
2	400	-2	2	0.8625	0.7625	0.8025
3	500	-2	2	0.85	0.775	0.80375
4	1000	-2	2	0.85	0.775	0.8137500000000001
6	2000	-2	2	0.85	0.7875	0.82
8	3000	-2	2	0.8625	0.8125	0.83375
}\kendallRiskOddRatio

\pgfplotstableread{
nz  dim ctxLeft ctxRight    max min ave
2	300	-2	2	0.8625	0.7375	0.8012499999999999
2	400	-2	2	0.875	0.775	0.8075000000000001
3	500	-2	2	0.85	0.7875	0.8087499999999999
4	1000	-2	2	0.8625	0.7875	0.8237500000000001
6	2000	-2	2	0.85	0.8	0.825
8	3000	-2	2	0.8625	0.8125	0.83375
}\kendalloddratioLiddel

==> weightings/kendallweighting.tex <==
\pgfplotstableread{
nz  dim ctxLeft ctxRight    max min ave
1	300	-2	2	0.8	0.725	0.760625
1	400	-2	2	0.8375	0.725	0.7743750000000003
1	500	-2	2	0.8625	0.75	0.7975000000000001
4	1000	-2	2	0.8375	0.7625	0.7949999999999998
2	2000	-2	2	0.875	0.775	0.8262499999999999
3	3000	-2	2	0.875	0.8	0.8300000000000001
}\kendalltscorePositiveOnly

\pgfplotstableread{
nz  dim ctxLeft ctxRight    max min ave
2	300	-2	2	0.8625	0.75	0.7975000000000001
2	400	-2	2	0.85	0.7625	0.8012499999999999
3	500	-2	2	0.85	0.775	0.8025
4	1000	-2	2	0.85	0.775	0.8137500000000001
6	2000	-2	2	0.85	0.7875	0.82
8	3000	-2	2	0.8625	0.8125	0.83375
}\kendallRelativeRisk

\pgfplotstableread{
nz  dim ctxLeft ctxRight    max min ave
1	300	-2	2	0.825	0.725	0.7724999999999999
1	400	-2	2	0.8625	0.725	0.7825
1	500	-2	2	0.8875	0.75	0.8074999999999999
1	1000	-2	2	0.8625	0.7125	0.8112500000000002
2	2000	-2	2	0.8875	0.775	0.8318750000000001
3	3000	-2	2	0.875	0.8	0.8418750000000002
}\kendallppmi

\pgfplotstableread{
nz  dim ctxLeft ctxRight    max min ave
1	300	-2	2	0.825	0.725	0.7724999999999999
1	400	-2	2	0.8625	0.725	0.7825
1	500	-2	2	0.8875	0.75	0.8074999999999999
1	1000	-2	2	0.8625	0.7125	0.8112500000000002
2	2000	-2	2	0.8875	0.775	0.8318750000000001
3	3000	-2	2	0.875	0.8	0.8418750000000002
}\kendallpmitwo

\pgfplotstableread{
nz  dim ctxLeft ctxRight    max min ave
2	300	-2	2	0.85	0.7375	0.7949999999999999
2	400	-2	2	0.8625	0.7625	0.7950000000000002
3	500	-2	2	0.8375	0.775	0.7962499999999999
4	1000	-2	2	0.85	0.775	0.81125
6	2000	-2	2	0.8375	0.7875	0.8125
8	3000	-2	2	0.85	0.8	0.82125
}\kendallliddel

\pgfplotstableread{
nz  dim ctxLeft ctxRight    max min ave
1	300	-2	2	0.7625	0.7125	0.735625
1	400	-2	2	0.775	0.7125	0.74
1	500	-2	2	0.825	0.675	0.7362500000000002
1	1000	-2	2	0.7625	0.675	0.71125
2	2000	-2	2	0.75	0.675	0.7125000000000001
3	3000	-2	2	0.775	0.6875	0.718125
}\kendalldice

\pgfplotstableread{
nz  dim ctxLeft ctxRight    max min ave
1	300	-2	2	0.7875	0.6875	0.730625
1	400	-2	2	0.775	0.675	0.7275
1	500	-2	2	0.7625	0.675	0.7099999999999999
1	1000	-2	2	0.725	0.65	0.6856250000000002
2	2000	-2	2	0.7125	0.6375	0.6749999999999999
3	3000	-2	2	0.7125	0.625	0.6812500000000001
}\kendalljakard

\pgfplotstableread{
nz  dim ctxLeft ctxRight    max min ave
2	300	-2	2	0.8625	0.7375	0.79625
2	400	-2	2	0.8625	0.7625	0.8025
3	500	-2	2	0.85	0.775	0.80375
4	1000	-2	2	0.85	0.775	0.8137500000000001
6	2000	-2	2	0.85	0.7875	0.82
8	3000	-2	2	0.8625	0.8125	0.83375
}\kendalloddratio


\pgfplotstableread{
nz  dim ctxLeft ctxRight    max min ave
2	300	-2	2	0.825	0.775	0.7825
2	400	-2	2	0.8125	0.775	0.7874999999999999
3	500	-2	2	0.8125	0.775	0.79375
4	1000	-2	2	0.8125	0.7875	0.8012499999999999
6	2000	-2	2	0.825	0.75	0.7962499999999999
8	3000	-2	2	0.825	0.8	0.8087499999999999
}\kendallzscore


\pgfplotstableread{
nz  dim ctxLeft ctxRight    max min ave
2	300	-2	2	0.85	0.7375	0.7874999999999999
2	400	-2	2	0.8125	0.7375	0.7875000000000001
3	500	-2	2	0.825	0.7875	0.7987499999999998
4	1000	-2	2	0.825	0.7625	0.7975000000000001
6	2000	-2	2	0.825	0.775	0.8012499999999999
8	3000	-2	2	0.8375	0.8	0.8087500000000001
}\kendalltscor

\pgfplotstableread{
nz  dim ctxLeft ctxRight    max min ave
2	300	-2	2	0.8625	0.75	0.7987500000000001
2	400	-2	2	0.8625	0.7625	0.8025
3	500	-2	2	0.85	0.775	0.8025
4	1000	-2	2	0.85	0.775	0.8137500000000001
6	2000	-2	2	0.85	0.7875	0.82
8	3000	-2	2	0.8625	0.8125	0.83375
}\kendallpmi

==> weightings/pearsonweightins.tex <==
% Alternative: inline table data:
\pgfplotstableread{
nz  dim ctxLeft ctxRight    max min ave
1	300	-2	2	0.825	0.7	0.7549999999999998
1	400	-2	2	0.825	0.725	0.78
1	500	-2	2	0.85	0.7375	0.78625
1	1000	-2	2	0.85	0.7625	0.8175
2	2000	-2	2	0.8625	0.7875	0.8179166666666667
3	3000	-2	2	0.8625	0.7875	0.8275
4	4000	-2	2	0.825	0.7875	0.8108333333333333
}\pearsonwppmi

\pgfplotstableread{
nz  dim ctxLeft ctxRight    max min ave
1	300	-2	2	0.825	0.7125	0.7581250000000002
1	400	-2	2	0.8125	0.7125	0.7681250000000001
1	500	-2	2	0.825	0.7125	0.77125
1	1000	-2	2	0.825	0.75	0.7887500000000001
2	2000	-2	2	0.825	0.7625	0.7925
3	3000	-2	2	0.825	0.75	0.7918749999999999
}\pearsonwppmitwo

\pgfplotstableread{
nz  dim ctxLeft ctxRight    max min ave
1	300	-2	2	0.8125	0.7	0.7518750000000001
1	400	-2	2	0.8	0.7	0.756875
1	500	-2	2	0.7875	0.7125	0.7537499999999999
1	1000	-2	2	0.8125	0.7125	0.7724999999999999
2	2000	-2	2	0.8	0.75	0.7775
3	3000	-2	2	0.8125	0.7375	0.7799999999999999
}\pearsonwppmithree

\pgfplotstableread{
nz  dim ctxLeft ctxRight    max min ave
1	300	-2	2	0.825	0.7125	0.758125
1	400	-2	2	0.8125	0.725	0.7762500000000001
1	500	-2	2	0.85	0.7375	0.78625
1	1000	-2	2	0.85	0.775	0.8156249999999998
2	2000	-2	2	0.8625	0.7875	0.8174999999999999
3	3000	-2	2	0.8625	0.7875	0.8200000000000001
}\positiveRelativeRiskLog

\pgfplotstableread{
nz  dim ctxLeft ctxRight    max min ave
1	300	-2	2	0.7625	0.6	0.6687500000000001
1	400	-2	2	0.75	0.6125	0.69
1	500	-2	2	0.75	0.6375	0.698125
1	1000	-2	2	0.7875	0.625	0.7225
2	2000	-2	2	0.8125	0.7125	0.7493750000000001
3	3000	-2	2	0.8	0.725	0.7637499999999998
}\liddel

\pgfplotstableread{
nz  dim ctxLeft ctxRight    max min ave
1	300	-2	2	0.7375	0.6	0.6668749999999999
1	400	-2	2	0.7125	0.5875	0.64625
1	500	-2	2	0.7125	0.5875	0.6456250000000001
1	1000	-2	2	0.7125	0.575	0.6518750000000001
2	2000	-2	2	0.725	0.6125	0.654375
3	3000	-2	2	0.75	0.6	0.6581249999999998
}\jaccard

\pgfplotstableread{
nz  dim ctxLeft ctxRight    max min ave
1	300	-2	2	0.825	0.7125	0.7575000000000001
1	400	-2	2	0.8125	0.725	0.776875
1	500	-2	2	0.85	0.7375	0.78625
1	1000	-2	2	0.85	0.7625	0.8149999999999998
2	2000	-2	2	0.8625	0.7875	0.8162499999999998
3	3000	-2	2	0.8625	0.7875	0.8187500000000002
}\oddratiologpos


